Is my Driver Observation Model Overconfident? Input-guided Calibration Networks for Reliable and Interpretable Confidence Estimates

Driver observation models are rarely deployed under perfect conditions. In practice, illumination, camera placement and type differ from the ones present during training and unforeseen behaviours may occur at any time. While observing the human behind the steering wheel leads to more intuitive human-vehicle-interaction and safer driving, it requires recognition algorithms which do not only predict the correct driver state, but also determine their prediction quality through realistic and interpretable confidence measures. Reliable uncertainty estimates are crucial for building trust and are a serious obstacle for deploying activity recognition networks in real driving systems. In this work, we for the first time examine how well the confidence values of modern driver observation models indeed match the probability of the correct outcome and show that raw neural network-based approaches tend to significantly overestimate their prediction quality. To correct this misalignment between the confidence values and the actual uncertainty, we consider two strategies. First, we enhance two activity recognition models often used for driver observation with temperature scaling-an off-the-shelf method for confidence calibration in image classification. Then, we introduce Calibrated Action Recognition with Input Guidance (CARING)-a novel approach leveraging an additional neural network to learn scaling the confidences depending on the video representation. Extensive experiments on the Drive&Act dataset demonstrate that both strategies drastically improve the quality of model confidences, while our CARING model out-performs both, the original architectures and their temperature scaling enhancement, leading to best uncertainty estimates.

==> tables/tbl_results_class_wise_ece_old.tex <==
%!TEX root = ../root.tex



\begin{table*}[]
%\begin{table*}[!htbp]
	\centering
	\scalebox{1.1}{
\begin{tabular}{ll|lll|lll}
	\toprule
	Annotation                                   & Recall   & MeanScore & DeltaAcc & ECE     & MeanScore & DeltaAcc & ECE     \\
	\midrule
	closing bottle                              & 67.65  & 88.97   & 21.33  & 24.12 & 68.39   & .74    & 12.62 \\
	closing door inside                        & 92.31  & 98.51   & 6.21   & 8.22  & 86.00   & -6.31  & 8.30  \\
	closing door outside                       & 81.82  & 93.55   & 11.73  & 20.97 & 86.86   & 5.04   & 19.81 \\
	closing laptop                              & 53.85  & 87.52   & 33.67  & 35.96 & 65.41   & 11.57  & 21.71 \\
	drinking                                     & 81.69  & 96.62   & 14.93  & 16.41 & 90.32   & 8.63   & 11.63 \\
	eating                                       & 86.42  & 93.26   & 6.84   & 9.33  & 80.99   & -5.43  & 5.75  \\
	entering car                                & 100.00 & 99.25   & -.75   & .75   & 91.31   & -8.69  & 8.69  \\
	exiting car                                 & 100.00 & 95.17   & -4.83  & 4.83  & 91.19   & -8.81  & 8.81  \\
	fastening seat belt                        & 90.00  & 96.08   & 6.08   & 6.91  & 88.36   & -1.64  & 7.24  \\
	fetching an object                         & 76.03  & 93.77   & 17.74  & 18.28 & 79.42   & 3.40   & 5.32  \\
	interacting with phone                     & 85.49  & 96.04   & 10.55  & 10.55 & 84.67   & -.82   & 3.28  \\
	looking or moving around  & 16.13  & 88.29   & 72.16  & 72.16 & 66.47   & 50.34  & 50.34 \\
	opening backpack                            & .00    & 98.82   & 98.82  & 98.82 & 82.69   & 82.69  & 82.69 \\
	opening bottle                              & 58.54  & 89.74   & 31.21  & 34.87 & 73.73   & 15.20  & 23.12 \\
	opening door inside                        & 81.25  & 93.51   & 12.26  & 12.26 & 81.18   & -.07   & 10.20 \\
	opening door outside                       & 100.00 & 100.00  & .00    & .00   & 98.16   & -1.84  & 1.84  \\
	opening laptop                              & 57.89  & 83.18   & 25.28  & 30.23 & 59.23   & 1.33   & 25.52 \\
	placing an object                          & 66.77  & 93.03   & 26.25  & 26.25 & 75.90   & 9.13   & 9.25  \\
	preparing food                              & 5.00   & 90.01   & 85.01  & 85.01 & 61.51   & 56.51  & 56.51 \\
	pressing automation button                 & 88.17  & 98.68   & 10.51  & 11.06 & 91.80   & 3.63   & 5.20  \\
	putting laptop into backpack              & 16.67  & 92.67   & 76.00  & 76.00 & 76.46   & 59.80  & 59.80 \\
	putting on jacket                          & 54.44  & 87.38   & 32.93  & 32.93 & 66.25   & 11.81  & 15.92 \\
	putting on sunglasses                      & 75.00  & 95.29   & 20.29  & 20.29 & 85.89   & 10.89  & 13.48 \\
	reading magazine                            & 92.93  & 98.58   & 5.65   & 6.09  & 93.35   & .42    & 2.87  \\
	reading newspaper                           & 94.47  & 97.32   & 2.85   & 4.19  & 87.68   & -6.79  & 7.40  \\
	sitting still                               & 95.10  & 97.96   & 2.86   & 2.86  & 93.84   & -1.26  & 1.84  \\
	taking laptop from backpack               & .00    & 85.25   & 85.25  & 85.25 & 70.08   & 70.08  & 70.08 \\
	taking off jacket                          & 60.00  & 86.68   & 26.68  & 31.75 & 64.15   & 4.15   & 17.50 \\
	taking off sunglasses                      & 41.18  & 88.05   & 46.87  & 46.87 & 68.86   & 27.68  & 29.20 \\
	talking on phone                           & 71.60  & 92.55   & 20.95  & 22.96 & 78.26   & 6.65   & 13.36 \\
	unfastening seat belt                      & 80.56  & 91.89   & 11.34  & 12.77 & 77.44   & -3.11  & 13.82 \\
	using multimedia display                   & 92.39  & 97.38   & 4.99   & 4.99  & 91.25   & -1.14  & 2.28  \\
	working on laptop                          & 86.86  & 94.33   & 7.48   & 9.51  & 85.67   & -1.19  & 3.89  \\
	writing                                      & 86.07  & 95.03   & 8.97   & 11.51 & 85.19   & -.88   & 3.39  \\
	\midrule
	Mean                                         & 68.71  & 93.36   & 24.65  & 26.32 & 80.23   & 11.52  & 18.61\\
\bottomrule

\end{tabular}
	}
	\caption{
	Fine-grained activity level results for different views and modalities and their combination (I3D model). 	
		%Fine-grained Activities Recognition results for all views for I3D. Random Baseline accuracy is $2.94$.
	% We show that even though the driver is mostly visible in the frame for each of our selected views, the camera position still plays an important role in the performance of our models. 
	}
	\label{tbl:class-wise}
	\vspace{-0.3cm}
	
\end{table*}

==> tables/tbl_results_reliability.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table}[b]
	\scalebox{0.72}{
	\begin{tabular}{ @{}l|cc|cc|cc|cc@{}}
		\toprule
		\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \multicolumn{2}{c|}{\textbf{NLL}} & \multicolumn{2}{c}{\textbf{$\Delta_{Acc}$}} \\
		& val & test & val & test & val & test & val & test \\ 
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} \\
		I3D \cite{carreira2017quo} & 20.1 & X & X & X & X & X & X & X \\
		P3D & X & X & X & X & X & X & X & X \\
		C3D & X & X & X & X & X & X & X & X \\
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}\\
		I3D + Temperature Scaling \cite{Guo2017} &	4.00& 7.75 & 26.08 & 17.34 & 0.81 &1.57& X & X \\
		CARING - I3D w.o. shuffle loss & 2.89 & 6.11 &  18.75 & 14.80 & 0.81 & 1.54 & X & X \\
		CARING - I3D  & 2.72 & 6.02 &  14.23 & 13.12 & 0.82  & 1.54 & X & X \\

%		\bottomrule

	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	\vspace{-0.3cm}
	\label{table:action_reco_objectlevel}
	
	
	

\end{table}



==> tables/tbl_results_reliability_hmdb51.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table}[b]
	\scalebox{0.72}{
	\begin{tabular}{ @{}l|cc|cc|cc|cc@{}}
		\toprule
		\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{ECE}} & \multicolumn{2}{c|}{\textbf{MCE}} & \multicolumn{2}{c|}{\textbf{NLL}} & \multicolumn{2}{c}{\textbf{$\Delta_{Acc}$}} \\
		& val & test & val & test & val & test & val & test \\ 
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} \\
		I3D \cite{carreira2017quo} & 20.1 & X & X & X & X & X & X & X \\
		P3D & X & X & X & X & X & X & X & X \\
		C3D & X & X & X & X & X & X & X & X \\
		\midrule
		\multicolumn{9}{l}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}\\
		I3D + Temperature Scaling \cite{Guo2017} &	4.00& 7.75 & 26.08 & 17.34 & 0.81 &1.57& X & X \\
		CARING - I3D w.o. shuffle loss & 2.89 & 6.11 &  18.75 & 14.80 & 0.81 & 1.54 & X & X \\
		CARING - I3D  & 2.72 & 6.02 &  14.23 & 13.12 & 0.82  & 1.54 & X & X \\

%		\bottomrule

	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	\vspace{-0.3cm}
	\label{table:action_reco_objectlevel}
	
	
	

\end{table}



==> tables/tbl_results_reliability_multi_view_old.tex <==
%!TEX root = ../root.tex


\begin{table*}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccc|cccccccc|cccccccc}
\toprule
Model & \multicolumn{8}{c}{Rare classes} & \multicolumn{8}{c}{Common classes} & \multicolumn{8}{c}{All classes} \\
 & \multicolumn{2}{c}{ECE} & \multicolumn{2}{c}{MCE} & \multicolumn{2}{c}{NLL} & \multicolumn{2}{c}{Acc} & \multicolumn{2}{c}{ECE} & \multicolumn{2}{c}{MCE} & \multicolumn{2}{c}{NLL} & \multicolumn{2}{c}{Acc} & \multicolumn{2}{c}{ECE} & \multicolumn{2}{c}{MCE} & \multicolumn{2}{c}{NLL} & \multicolumn{2}{c}{Acc} \\
 & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} & \multicolumn{1}{c}{val} & \multicolumn{1}{c}{test} \\
 \midrule
\textbf{Front top NIR (ids 1)} & & & & & & & & & & & & & & & & & & & &      & & & \\
Raw 3D CNN &31.48 & 43.32 & 75.04& 69.66& 3.41 & 4.54 & & & 10.22 & 13.38   & 66.59  & 40.05  & 0.90 & 1.27 &  &  & 11.72 & 15.98  & 66.47  & 40.18     & 0.90 & 1.56& & \\
Temp. Scaling & 24.97 & 32.38 & 71.74 & 58.94 & 1.96 & 2.62 & &  & 5.31  & 6.99& 56.27 & 23.37& 0.57 & 0.83 &  & & 6.59  & 8.55 & 48.93 & 24.95 & 0.68 & 0.99& & \\
CARING  & 18.34 & 23.60 & 52.05  & 50.91 & 1.55 & 2.17  & &  & 2.57  & 6.22  & 63.42& 22.43& 0.50 & 0.78  & &  & 3.04  & 6.02& 46.42 & 20.33              & 0.58 & 0.90 & &   \\ 
 \midrule
\textbf{Right top NIR (ids 2)} & & &  & & &  & &  & & & & & & & & & & & & & &  &  & \\
Raw 3D CNN  & 35.89 & 42.86 & 81.20 & 77.86 & 3.79 & 4.78  &  && 14.73 & 15.83 & 43.36& 36.28  & 1.28 & 1.42  & &  & 16.26 & 18.23 & 45.74  & 40.02 & 1.48 & 1.73  & &\\
Temp. Scaling  & 25.69 & 29.52 & 66.00 & 59.70& 2.20 & 2.73 & &  & 6.59  & 6.57 & 25.36 & 25.15 & 0.82 & 0.93 &  & & 7.71  & 7.97 & 26.42 & 26.85 & 0.93 & 1.10 &  &  \\
CARING   & 20.49 & 24.03 & 62.99 & 59.36  & 1.92 & 2.39  &     & & 3.39  & 5.30 & 15.43 & 22.83  & 0.76 & 0.90  & & & 3.67  & 5.67  & 15.18 & 17.30& 0.85 & 1.03  & &  \\
\midrule
\textbf{Back NIR (ids 3) } & & & & & & &  & & & & & & & &     & & & & & & & & &\\
Raw 3D CNN& 40.17 & 49.47 & 69.32 & 76.45 & 0.44 & 5.23 &     & & 16.07 & 19.55 & 55.69 & 54.60 & 1.58 & 1.67 & & & 17.85 & 22.14& 55.10  & 62.81 & 4.42 & 2.00 & & \\
Temp. Scaling & 25.45 & 33.69 & 74.12 & 76.62 & 0.27 & 3.00&   & & 5.19  & 9.00 & 34.35 & 23.89 & 1.14 & 1.06 & & & 6.03  & 11.00 & 27.85 & 29.20 & 1.26 & 1.24 & & \\
CARING  & 19.95 & 26.58 & 71.97 & 67.14 & 0.24 & 2.67& & & 3.48 & 5.25 & 19.58 & 26.69 & 1.07 & 1.01 & & & 3.17 & 6.59  & 17. & 41.06 & 1.17 & 1.16 & & \\ 
 \midrule
\textbf{Face View NIR (4)}& & & & & & & & & & & & & & & & & & & & & & & &\\
Raw 3D CNN  & 39.22 & 45.56 & 76.01& 74.18  & 4.60 & 4.97      & &  & 19.89 & 21.40 & 33.53  & 37.20   & 2.02 & 2.02         & &  & 21.34 & 23.50 & 35.18& 38.92 & 2.22 & 2.28 &  & \\
Temp. Scaling& 24.76 & 26.14 & 67.62& 67.74   & 2.59 & 3.03    & & & 6.30 & 6.68 & 13.98 & 12.98 & 1.39 & 1.53 & & & 6.78  & 6.81 & 14.84& 11.51& 1.48 & 1.67& & \\
CARING & 18.93 & 23.20 & 57.42 & 57.70 & 2.37 & 2.94 & &  & 4.22 & 10.32 & 24.34 & 20.68 & 1.27 & 1.53 & & & 4.63 & 9.87 & 24.37 & 20.24 & 1.36 & 1.66& &\\ 
 \midrule
\textbf{Left top NIR (5)} & & & & & & & & & & & & & & & & & & & & & & & &\\
Raw 3D CNN & 31.17 & 44.11 & 79.39  & 77.75& 2.96 & 4.23  &  && 9.43  & 12.43  & 47.52 & 48.63& 0.92 & 1.18&&& 11.10 & 15.16& 50.11 & 49.57 & 1.08 & 1.46 &  &\\
Temp. Scaling                  & 21.46 & 31.12 & 64.22  & 76.87& 1.79 & 2.58 && & 4.96  & 6.23 & 24.13  & 25.09 & 0.59 & 0.83 & & & 5.88  & 7.69  & 25.43 & 38.13 & 0.69 & 0.99 &  &  \\
CARING                         & 18.14 & 25.46           & 68.09                   & 63.49                    & 1.53 & 2.34             &     &                          & 2.45  & 6.58            & 21.34                   & 21.91                    & 0.49 & 0.82             &     &                          & 2.95  & 5.77            & 25.52                   & 37.70                    & 0.57 & 0.97             &     &                    \\ 
 \midrule
\textbf{Kinect IR}             &       &                 &                         &                          &      &                  &     &                          &       &                 &                         &                          &      &                  &     &                          &       &                 &                         &                          &      &                  &     &                    \\
Raw 3D CNN                     & 29.65 & 36.12           & 72.45                   & 68.25                    & 3.03 & 3.69             &     &                          & 80.45 & 13.69           & 44.55                   & 36.13                    & 0.84 & 1.253            &     &                          & 9.51  & 15.67           & 44.37                   & 37.41                    & 1.01 & 1.48             &     &                    \\
Temp. Scaling                  & 20.81 & 23.88           & 74.03                   & 61.08                    & 2.00 & 2.38             &     &                          & 49.95 & 6.17            & 52.61                   & 38.96                    & 0.64 & 0.89             &     &                          & 5.11  & 7.49            & 41.69                   & 28.32                    & 0.74 & 1.03             &     &                    \\
CARING                         & 15.66 & 19.90           & 63.68                   & 60.65                    & 1.78 & 2.20             &     &                          & 2.81  & 5.19            & 18.97                   & 17.89                    & 0.53 & 0.85             &     &                          & 2.69  & 6.16            & 16.70                   & 17.06                    & 0.63 & 0.97             &     &                    \\ 
 \midrule
textbf{Kinect Depth}          &       &                 &                         &                          &      &                  &     &                          &       &                 &                         &                          &      &                  &     &                          &       &                 &                         &                          &      &                  &     &                    \\
Raw 3D CNN                     & 32.43 & 41.69           & 77.73                   & 77.30                    & 3.23 & 4.44             &     &                          & 11.72 & 16.83           & 57.95                   & 39.30                    & 1.01 & 1.51             &     &                          & 13.13 & 18.94           & 44.70                   & 42.20                    & 1.17 & 1.78             &     &                    \\
Temp. Scaling                  & 23.88 & 29.36           & 69.89                   & 63.75                    & 1.94 & 2.66             &     &                          & 4.93  & 6.81            & 19.44                   & 24.12                    & 0.70 & 1.03             &     &                          & 5.82  & 8.32            & 19.70                   & 26.75                    & 0.80 & 1.18             &     &                    \\
CARING                         & 18.84 & 25.05           & 68.76                   & 57.53                    & 1.67 & 2.35             &     &                          & 3.08  & 5.00            & 17.90                   & 37.50                    & 0.65 & 0.97             &     &                          & 3.44  & 5.50            & 15.92                   & 36.54                    & 0.72 & 1.10             &     &                    \\ 
 \midrule
\textbf{Kinect Color}          &       &                 &                         &                          &      &                  &     &                          &       &                 &                         &                          &      &                  &     &                          &       &                 &                         &                          &      &                  &     &                    \\
Raw 3D CNN                     & 28.00 & 40.38           & 73.15                   & 67.72                    & 3.14 & 4.66             &     &                          & 9.80  & 13.21           & 42.08                   & 56.66                    & 0.98 & 1.20             &     &                          & 8.99  & 15.56           & 41.25                   & 58.48                    & 1.14 & 1.51            &     &                    \\
Temp. Scaling                  & 21.47 & 31.06           & 57.75                   & 62.68                    & 1.80 & 2.66             &     &                          & 4.93  & 7.64            & 22.06                   & 28.52                    & 0.60 & 0.78             &     &                          & 5.86  & 9.43            & 19.01                   & 27.13                    & 0.69 & 0.95           &     &                    \\
CARING                         & 15.88 & 24.10           & 59.09                   & 56.00                    & 1.80 & 2.21             &     &                          & 2.73  & 6.10            & 17.17                   & 27.58                    & 0.51 & 0.74             &     &                          & 3.08  & 6.54            & 14.89                   & 29.03                    & 0.59 & 0.87            &     &                    \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/tbl_results_reliability_pakos_ids1_ids1.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table*}[b]
	\scalebox{0.78}{
	\begin{tabular}{ l|cccccc|cccccc|cccccc}
		%\specialrule{.8pt}{2pt}{0pt}
		\toprule
		\multirow{3}{*}{\cellcolor{tablegrey} \textbf{Model}}& \multicolumn{6}{c|}{\cellcolor{lightsteellila}\textbf{All activity classes}} & \multicolumn{6}{c|}{\cellcolor{lightsteelblue} \textbf{Rare activity classes}} & \multicolumn{6}{c}{\cellcolor{lightsteelgreen} \textbf{Common activity classes}}\\ 
		 \cellcolor{tablegrey} \textbf{Model}&\multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{ECE}} &
		 \multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteellila}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteelblue}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{MCE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{NLL}} \\
		\cellcolor{tablegrey}&\cellcolor{lightsteellila} val &\cellcolor{lightsteellila} test &\cellcolor{lightsteellila} val & \cellcolor{lightsteellila}test & \cellcolor{lightsteellila}val & \cellcolor{lightsteellila}test  &\cellcolor{lightsteelblue} val &\cellcolor{lightsteelblue} test & \cellcolor{lightsteelblue}val &\cellcolor{lightsteelblue}test &\cellcolor{lightsteelblue} val & \cellcolor{lightsteelblue}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test & \cellcolor{lightsteelgreen}val & \cellcolor{lightsteelgreen}test  \\ 
		\specialrule{.4pt}{0pt}{2pt}
		%\hline
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} & & & & & & & & & & & & \\
		I3D \cite{carreira2017quo} & 13.68 & 15.95 & 50.95 &  49.08 & 1.05 & 1.31 & & & & & & & & & & & & \\
		P3D & X & X & X & X & X & X  & & & & & & & & & & & & \\
		%C3D & X & X & X & X & X & X  \\
		\midrule
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}& & & & & & & & & & & & \\
		I3D + Temperature Scaling \cite{Guo2017} &	7.12& 7.57 & 32.50 & 21.73 & 0.75 &0.96 & & & & & & & & & & & & \\
		CARING - I3D  & 5.12 & 6.95 & 26.87  & 46.38 & 0.73 & 0.94  & & & & & & & & & & & & \\


& & & & & & & & & & & &  \\
		\bottomrule
	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	
	\label{table:action_reco_objectlevel}
	
	
	

\end{table*}



==> tables/tbl_results_reliability_pakos_ids1_ids1_wide.tex <==
%!TEX root = ../root.tex



%\begin{table}[!htbp]
\begin{table*}[b]
	\scalebox{0.78}{
	\begin{tabular}{ l|cccccc|cccccc|cccccc}
		%\specialrule{.8pt}{2pt}{0pt}
		\toprule
		\multirow{3}{*}{\cellcolor{tablegrey} \textbf{Model}}& \multicolumn{6}{c|}{\cellcolor{lightsteellila}\textbf{All activity classes}} & \multicolumn{6}{c|}{\cellcolor{lightsteelblue} \textbf{Rare activity classes}} & \multicolumn{6}{c}{\cellcolor{lightsteelgreen} \textbf{Common activity classes}}\\ 
		 \cellcolor{tablegrey} \textbf{Model}&\multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{ECE}} &
		 \multicolumn{2}{c}{\cellcolor{lightsteellila}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteellila}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelblue}\textbf{MCE}} & \multicolumn{2}{c|}{\cellcolor{lightsteelblue}\textbf{NLL}}&
		 \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{ECE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{MCE}} & \multicolumn{2}{c}{\cellcolor{lightsteelgreen}\textbf{NLL}} \\
		\cellcolor{tablegrey}&\cellcolor{lightsteellila} val &\cellcolor{lightsteellila} test &\cellcolor{lightsteellila} val & \cellcolor{lightsteellila}test & \cellcolor{lightsteellila}val & \cellcolor{lightsteellila}test  &\cellcolor{lightsteelblue} val &\cellcolor{lightsteelblue} test & \cellcolor{lightsteelblue}val &\cellcolor{lightsteelblue}test &\cellcolor{lightsteelblue} val & \cellcolor{lightsteelblue}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test &\cellcolor{lightsteelgreen} val & \cellcolor{lightsteelgreen}test & \cellcolor{lightsteelgreen}val & \cellcolor{lightsteelgreen}test  \\ 
		\specialrule{.4pt}{0pt}{2pt}
		%\hline
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Conventional Action Recognition Models}} & & & & & & & & & & & & \\
		I3D \cite{carreira2017quo} & 13.68 & 15.95 & 50.95 &  49.08 & 1.05 & 1.31 & & & & & & & & & & & & \\
		P3D & X & X & X & X & X & X  & & & & & & & & & & & & \\
		%C3D & X & X & X & X & X & X  \\
		\midrule
		\multicolumn{7}{l|}{\hspace{-6pt}\textbf{Uncertainty-calibrated Models}}& & & & & & & & & & & & \\
		I3D + Temperature Scaling \cite{Guo2017} &	7.12& 7.57 & 32.50 & 21.73 & 0.75 &0.96 & & & & & & & & & & & & \\
		CARING - I3D  & 5.12 & 6.95 & 26.87  & 46.38 & 0.73 & 0.94  & & & & & & & & & & & & \\


& & & & & & & & & & & &  \\
		\bottomrule
	\end{tabular}
		}
	\caption{Recognition of Atomic Action Units defined as \textit{\{Action, Object, Location\}} triplets. 	
	% We show the accuracy of each element in the triplet when evaluated separately.
	% In the last column, we include the accuracy of the triplets where we evaluate all three values together. 
	}
	
	\label{table:action_reco_objectlevel}
	
	
	

\end{table*}


